A Rewriting Logic Approach to Specification, Proof-search, and Meta-proofs in Sequent Systems

This paper develops an algorithmic-based approach for proving inductive properties of propositional sequent systems such as admissibility, invertibility, cut-elimination, and identity expansion. Although undecidable in general, these structural properties are crucial in proof theory because they can reduce the proof-search effort and further be used as scaffolding for obtaining other meta-results such as consistency. The algorithms -- which take advantage of the rewriting logic meta-logical framework, and use rewrite- and narrowing-based reasoning -- are explained in detail and illustrated with examples throughout the paper. They have been fully mechanized in the L-Framework, thus offering both a formal specification language and off-the-shelf mechanization of the proof-search algorithms coming together with semi-decision procedures for proving theorems and meta-theorems of the object system. As illustrated with case studies in the paper, the L-Framework, achieves a great degree of automation when used on several propositional sequent systems, including single conclusion and multi-conclusion intuitionistic logic, classical logic, classical linear logic and its dyadic system, intuitionistic linear logic, and normal modal logics.

==> rew-id.tex <==
%!TEX root = main.tex
% !TEX spellcheck = en-US
The interface for this analysis is defined in \lstinline{id-expand.maude}:

\begin{lstlisting}

fth ID-EXP-SPEC is
  op mod-name : -> Qid .
  op file-name : -> String .
  op bound-spec : -> Nat .
  op goal : GroundTerm -> GroundTerm . --- ( F |-- F,  |- F, dual(F), etc)
  op already-proved-theorems : -> RuleSet .
  --- types different from 'Formula to be analyzed
  op types-formula : -> TypeList . 
endfth
\end{lstlisting}

The attribute  \code{goal} specifies the sequent to be proved. 
For instance, given a ground term formula $F$, in a two-sided (resp. one-sided) sequent system, it must return  $F \vdash F$
(resp. $\vdash F, F^\perp$ where $F^\perp$ denotes the dual of $F$  -- see Section \ref{ex:ll}). 

In the case of modal logics (Section \ref{case:modal}), additional subsort relations as \code{BFormula < Formula} are added to specify that boxed formulas ($\Box F$) are also formulas.The attribute \code{types-formula} lists such additional sorts (if any). 

The procedure 
builds a goal for each 
operators defined in the OL module of the form \code{op O : ... -> Ty} where \code{Ty} is either \code{'Formula} or it belongs to 
the list \code{types-formula}. 
A suitable definition 
\code{op inductive : GroundTerm -> RuleSet .} is used to produce the needed inductive hypothesis (on smaller formulas). 

==> thealgo.tex <==
\begin{algorithm}[t]
\KwIn{\lstinline{M : Module *** system of rules}

\quad\qquad\   \lstinline{Th : Rule *** theorem to be proved}
}
    
\KwOut{ $\{  r\in rules(M) \mid \mbox{ $Th$ holds in $r$}\}$}

\Begin{
  $result := \emptyset$
 
 \ForEach{$r \in rules(M)$}{
  $check := true$
 
 \ForEach{$\theta \in unify(head(r), head(Th))$}{
  $T := head(r) \theta$
 
 \ForEach{$T_R \in apply(T, r)$}{
    $IH := \{T_R\} \cup apply(Tr, Th)$
   
    \ForEach{$goal \in  rewrite(T,Th)$}{
   
    $M' := M \cup \{ t \Rightarrow proved \mid t \in IH\}$
   
   \lIf{  $not (M' \vdash goal \Rightarrow^* proved)$}{$check := false$}
   }
 }
 }
  \lIf{check}{$result := result \cup \{r\}$}
  } %end FPR
}
 \caption{Proving that theorem $Th$ holds for the system $M$. \label{alg:prover}}
\end{algorithm}


